Load-Balanced Sparse MTTKRP on GPUs

Sparse matricized tensor times Khatri-Rao product (MTTKRP) is one of the most computationally expensive kernels in sparse tensor computations. This work focuses on optimizing the MTTKRP operation on GPUs, addressing both performance and storage requirements. We begin by identifying the performance bottlenecks in directly extending the state-of-the-art CSF (compressed sparse fiber) format from CPUs to GPUs. A significant challenge with GPUs compared to multicore CPUs is that of utilizing the much greater degree of parallelism in a load-balanced fashion for irregular computations like sparse MTTKRP. To address this issue, we develop a new storage-efficient representation for tensors that enables high-performance, load-balanced execution of MTTKRP on GPUs. A GPU implementation of sparse MTTKRP using the new sparse tensor representation is shown to outperform all currently known parallel sparse CPU and GPU MTTKRP implementations.

==> code/CSFGPUaldo.tex <==
\begin{algorithm}[h!]
\footnotesize
% \color{gray}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKw{To} {\textbf{to}}
    \SetKw{Step} {\textbf{step}}
    \SetKw{In} {\textbf{in}}
    \SetKw{return} {\textbf{return}}

    \Input{$~$ slicePtr, sliceIdx, fiberPtr, fiberIdx, X[2], dense matrices A[I][F], B[J][F], C[K][F]}
    \Output{$~$ dense matrix $Y$[I][F]}
    warpPerSlice = 

    \BlankLine
    \For{slc = 0 \To I} {
    	i = sliceIdx[slc] \\
        \For{fbr = slicePtr[slc] \To slicePtr[slc + 1]} {
    	j = fiberIdx[fbr] \\
            \For{idx = fiberPtr[fbr] \To fiberPtr[fbr + 1]} {
    	       k = X[2][idx] \\   
     	       \For{r = 0 \To R} {
    		        tmp[r] += Xval[idx] * C[k][r] \\
    		    }
    	   }
            \For{r = 0 \To R} {
                $Y$[i][r] += tmp[r] * B[j][r]
            }
        }
    }
	\return $Y$
    % P[ind] = val[ind] * sum \\
\caption{cuCSF-MTTKRP on GPU for 3D tensors}
\label{algo:CSF}
\end{algorithm} 

